Interpolating between Optimal Transport and MMD using Sinkhorn Divergences

Comparing probability distributions is a fundamental problem in data sciences. Simple norms and divergences such as the total variation and the relative entropy only compare densities in a point-wise manner and fail to capture the geometric nature of the problem. In sharp contrast, Maximum Mean Discrepancies (MMD) and Optimal Transport distances (OT) are two classes of distances between measures that take into account the geometry of the underlying space and metrize the convergence in law. This paper studies the Sinkhorn divergences, a family of geometric divergences that interpolates between MMD and OT. Relying on a new notion of geometric entropy, we provide theoretical guarantees for these divergences: positivity, convexity and metrization of the convergence in law. On the practical side, we detail a numerical scheme that enables the large scale application of these divergences for machine learning: on the GPU, gradients of the Sinkhorn loss can be computed for batches of a million samples.

==> sections/numerics-OLD.tex <==
% !TEX root = ../AISTATS-Sinkhorn.tex


\section{Experiments}
\subsection{Numerical understanding}
Optimal Transport distances are non trivial objects which deserve a study of their numerical behaviour. We show in this section their performance with comparisons to kernel norms (i.e. MMD) in contexts of shape registration and computation of gradients. The properties of gradients are fundamental in order to optimize any model's parameters (e.g. a neural network).


\begin{figure}[b!]
    \centering
    
    \begin{subfigure}[t]{.6\linewidth}
		\centering
		\includegraphics[width=\linewidth]{sections/images/moons_hausdorff_L1_S_10its.png}
		\caption{$\H_\epsilon(\al,\be)$.}
	\end{subfigure}
	
	\begin{subfigure}[t]{.6\linewidth}
		\centering
		\includegraphics[width=\linewidth]{sections/images/moons_sinkhorn_L1_S_100its.png}
		\caption{$\Wb_\epsilon(\al,\be)$.}
	\end{subfigure}
    
    \caption{ \textbf{A geometric intuition.}
    The lines from a measure to another are the ``mean springs''
        that drive the gradients of the Hausdorff and Sinkhorn
        loss
        The contour lines in the background denote the
        \emph{influence fields}, or \emph{dual potentials}. In (a), the red and blue lines
        picture $\a^{\al\leftrightarrow\al}$
        and $\b^{\be\leftrightarrow\be}$ respectively,
        while they stand for 
        $\a^{\al\rightarrow\be}$
        and $\b^{\be\rightarrow\al}$ 
        in (b) -- see 
        (\ref{eq:hausdorff_dual_potentials},
        \ref{eq:sinkhorn_dual_potentials}).
        \label{fig:hausdorff_vs_sinkhorn}}
\end{figure}


First let's only compare $\H_\epsilon$ and $\Wb_\epsilon$. Given two measures $(\al,\be)$, Figure~\ref{fig:hausdorff_vs_sinkhorn} shows the averaged direction of the gradient w.r.t. $\be$ on the support of $\al$, and vice versa. It roughly represent the way the reference measures will match on one another. We notice that the constraints of OT give to $\nabla\Wb_\epsilon$ directions which looks like a matching process, while $\nabla\H_\epsilon$ directs towards the closest neighbour, making it look like a projective metric. The properties of the gradient -- including the aforementioned remarks -- can be observed in Figures~(\ref{fig:flow_1D},\ref{fig:flow_2D}) which show the behaviour of a gradient flow towards a target measure. Various common metrics such as kernel MMD, Energy Distance or regularized OT are shown.

Those figures give precious insights on the properties of the chosen metrics and their gradients. All RBF kernel metrics --namely Gaussian and Laplacian kernels -- exhibits a "repulsive" effect, i.e. some points get further from the initial measure before approaching the target. However, all OT derived metrics -- Regularize OT, Hausdorff and Sinkhorn divergence --  and the MMD get always closer at each iteration of the flow. Kernel metrics' gradient vanish for points which are far from the target. Furthermore, RBF kernels produce gradients with negative signs, hence causing a repulsion from the target measure. Fortunately, MMD is a particular case of kernel metric whose gradient remains positive, though it still vanishes away from the target measure.

Another aspect is the one of bias. Indeed, concerning RBF kernels and Regularized OT, we observe that the final measure minimizing the cost is not the target measure, but a biased version of it. For instance we observe that the measure concentrates on the median for Regularized OT. In spite of the popularity of kernels in other tasks such as clustering, we see that they are not an efficient metric to match measures. Meanwhile, MMD, $\H_\epsilon$ and $\Wb_\epsilon$ all match the source to the target, which shows numerically that it is an unbiased measure of similarity between probability distributions. Besides, $\H_\epsilon$ exhibits a projective behaviour as oberved on Figure~\ref{fig:hausdorff_vs_sinkhorn}: in order to minimize the influence of the potential induced by the target measure, a slight amount of mass is moved abruptly on its support, and the rest of it moves smoothly towards the target. Such counter-natural effect encourages us to think that $\H_\epsilon$ is more an intermediate concept proving the positivity of $\Wb_\epsilon$ rather than a metric with relevant properties to compare measures.

\onecolumn
\begin{figure}[p]

\begin{minipage}{.69\columnwidth}
\caption{ Wasserstein gradient flows of $\al\mapsto \text{Loss}(\al,\be)$
on the real line. At time $t=\texttt{0}$,
$\al$ and $\be$ are uniform measures on $\texttt{[0,0.2]}$ and
$\texttt{[0.6,1]}$
sampled with 5,000 points each --
we display the density of $\al$ in red, and that of $\be$ in blue.
Then,
we display the density of $\al_t$ as it is
registered onto $\be$.\label{fig:flow_1D}}
\end{minipage}
\hfill
\begin{minipage}{.28\columnwidth}
\begin{tikzpicture}
\node[inner sep=0pt] (waffle) at (0,0)
    {\includegraphics[width=\textwidth]{sections/images/t0_1D.png}};
\node at (.7,.8) {at $t=\texttt{0.}$};
\end{tikzpicture}
\end{minipage}
Figures computed with an Earth-Mover's cost $\C(x,y)=|x-y|$
and a regularization strength or kernel scale
$\epsilon = \sigma = \texttt{.10}$.

\vspace{1cm}

\makebox[\textwidth][c]{
\begin{tikzpicture}
\node[inner sep=0pt] (waffle) at (0,0)
    {\includegraphics[width=0.8\textwidth]{sections/images/waffle_1D.png}};

\node at (-7.1,6.5) {\rotatebox{90}{Energy}};
\node at (-7.1,4) {\rotatebox{90}{Gaussian}};
\node at (-7.1,1.5) {\rotatebox{90}{Laplacian}};
\node at (-7.1,-1.3) {\rotatebox{90}{Reg. OT}};
\node at (-7.1,-4) {\rotatebox{90}{Hausdorff}};
\node at (-7.1,-6.5) {\rotatebox{90}{Sinkhorn}};


\node at (-5,8) {$t=\texttt{.25}$};
\node at (-1.6,8) {$t=\texttt{.50}$};
\node at (1.8,8) {$t=\texttt{1.00}$};
\node at (5.2,8) {$t=\texttt{5.00}$};
\end{tikzpicture}
}

\end{figure}



\begin{figure}[p]

\begin{minipage}{.69\columnwidth}
\caption{ Wasserstein gradient flows of $\al\mapsto \text{Loss}(\al,\be)$
on the 2D plane. 
This Figure is equivalent to Figure~\ref{fig:flow_1D},
albeit in dimension~2.
At time $t=\texttt{0}$,
$\al$ and $\be$ are measures in the unit square
sampled with 500 points each --
we display the samples of $\al$ in red, and those of $\be$ in blue.
Then,
we display the sampled measure $\al_t$ as it is
registered onto $\be$.\label{fig:flow_2D}}
\end{minipage}
\hfill
\begin{minipage}{.28\columnwidth}
\begin{tikzpicture}
\node[inner sep=0pt] (waffle) at (0,0)
    {\includegraphics[width=\textwidth]{sections/images/t0_2D.png}};
\node at (.3,2.) {at $t=\texttt{0.}$};
\end{tikzpicture}
\end{minipage}
Figures computed with an Earth-Mover's cost $\C(x,y)=\|x-y\|$
and a regularization strength or kernel scale
$\epsilon = \sigma = \texttt{.10}$, one tenth of the Figures' widths.

\vspace{1cm}

\makebox[\textwidth][c]{
\begin{tikzpicture}[scale=1]
\node[inner sep=0pt] (waffle) at (0,0)
    {\includegraphics[width=0.8\textwidth]{sections/images/waffle_2D.png}};

\node at (-7.1,6.5) {\rotatebox{90}{Energy}};
\node at (-7.1,4) {\rotatebox{90}{Gaussian}};
\node at (-7.1,1.5) {\rotatebox{90}{Laplacian}};
\node at (-7.1,-1.3) {\rotatebox{90}{Reg. OT}};
\node at (-7.1,-4) {\rotatebox{90}{Hausdorff}};
\node at (-7.1,-6.5) {\rotatebox{90}{Sinkhorn}};


\node at (-5,8) {$t=\texttt{.25}$};
\node at (-1.6,8) {$t=\texttt{.50}$};
\node at (1.8,8) {$t=\texttt{1.00}$};
\node at (5.2,8) {$t=\texttt{5.00}$};
\end{tikzpicture}
}

\end{figure}

\twocolumn

% \subsection{Numerical applications}


==> sections/preface.tex <==
% !TEX root = ../AISTATS-Sinkhorn.tex

\section*{Preface}

This report presents the results which were developed during my research internship on Optimal Transport at the mathematics department of the Ecole Normale Supérieure of Paris. The subject was to study the properties of the Sinkhorn divergence, which has recently been introduced as a similarity metric between measures derived from the theory of regularized optimal transport. The main purpose was to prove at which conditions such divergence would have properties which makes it a desirable metric for applications in machine learning. Such subject eventually became a collaboration with a PhD student from the department, Jean Feydy. He was motivated by the use of OT, since it naturally carries a geometric information. Thus, we collaborated on several contributions such as proving that the Sinkhorn divergence is positive and metrizes the convergence in law, demontrating needed properties of the regularized transport, or implementing it to draw illustrations of the metric's properties. I am currently trying to apply it to real ML data on a task where the use of optimal transport seems relevant.

This report is structured in two parts. The first one is a general introduction to Optimal Transport, from its origins to its applications. The second part is an early version of an article that will be submitted soon to a machine learning conference. It thus respects some of its constraints, such as the template or the number of pages. The main corpus presents the results needed to prove the importance of the Sinkhorn divergence, while the appendix offers complementary materials to understand deeper the theory of regularized optimal transport.


==> sections/wasserstein-old.tex <==
% !TEX root = ../AISTATS-Sinkhorn.tex

\section{Computational Optimal Transport}
\label{sec:ot}

\todo{Gab: this section should be shorten to only include the proof of the results used in the main text. }


The purpose of this appendix is to present some theoretical contributions on the regularity of regularized optimal transport, and give helpful details on the understanding on the concepts of Optimal Transport theory. We also aim at providing rigorous arguments on the properties of OT which have been admitted for sake of conciseness.

Note that as promised in section~\ref{sec:assumptions},
we now focus on probability measures $\al$ and $\be$ that
both belong to the set of \emph{unit mass}
positive measures $\Mm_1^+(\Xx)$.
We also assume that the ground cost $\C$ is a
Lipschitz function on the compact feature space $\Xx$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Regularized OT problems}
\label{sec:ot_problems}

\todo{Gab: I think this section can be removed.}

\paragraph{Primal ``Monge'' problem.}
Following~\cite{2016-genevay-nips}, we consider 
a regularized OT cost defined as
the sum of a \emph{linear} transportation cost
and an \emph{entropic} barrier of strength $\epsilon>0$.
The latter allows us to turn a (combinatorial) linear 
program on the simplex
into a smooth, tractable convex problem:
\begin{align} \hspace{-.3cm}
	\OT_\epsilon(\al,\be) &\eqdef
	\umin{\pi \in \mathcal{U}(\al,\be)}
	\langle \pi,\C\rangle 
	+ \epsilon \KL(\pi,\al\otimes\be)\\
		\mathcal{U}(\al,\be) &\eqdef \enscond{\pi \in \Mm_1^+(\Xx)}{
		\pi_1=\al, \pi_2=\be
		 }.
\end{align}
Here, we optimize on \emph{transport plans}
$\pi$ whose marginals $\pi_1$ and $\pi_2$
are respectively equal to $\al$ and $\be$.
The entropic regularization enforces
the absolute continuity of $\pi$
with respect to the tensor product $\al\otimes\be$:
there exists an $\al\otimes\be$-measurable function $p$
such that $\d\pi(x,y)=p(x,y)\d\al(x)\d\be(y)$,
and we can rewrite the problem as
\begin{align*}
\OT_\epsilon(\al,\be)=
&\min_{p:\Xx^2\rightarrow\R_{\geqslant0}} 
\int_{\Xx^2} p\C\d\al\d\be\\
&+ \epsilon \int_{\Xx^2} 
\big[ p\log(p) - p + 1 \big]\d\al\d\be
\end{align*}
under the constraint that
\begin{align*}
\int_\Xx p(x,y)\d\be(y)&=1
\text{\qquad\qquad for $\al$-a.e. $x$,}\\
\text{and\qquad\qquad}
\int_\Xx p(x,y)\d\al(x)&=1
\text{\qquad\qquad for $\be$-a.e. $y$.}
\end{align*}
If $\al$ and $\be$ both have finite support,
this problem can be implemented as a 
standard finite dimensional convex program
on the values of $p$.

\enlargethispage{2\baselineskip}


\begin{figure}[H]
\centering

\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\textwidth]{sections/images/wireframe_1.png}
\caption{OT plan from $\alpha$ to $\beta$.}
\end{subfigure}
\qquad
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\textwidth]{sections/images/matrix_1.png}
\caption{Seen as a matrix.}
\end{subfigure}
\medskip

\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\textwidth]{sections/images/wireframe_reg.png}
\caption{\emph{Entropized} plan from $\alpha$ to $\beta$.}
\end{subfigure}
\qquad
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\textwidth]{sections/images/matrix_reg.png}
\caption{Seen as a matrix.}
\end{subfigure}
\medskip

\caption{
\textbf{The Monge-Kantorovitch problem.}
Let $\al$ and $\be$ be two probability measures
in the 2D plane -- say, sampled curves.
(a) When $\epsilon=0$, 
the primal problem~\eqref{eq-primal-ot} is all about finding
a probabilistic mapping $\pi$ from $\al$ to $\be$
that minimizes the average displacement cost $\langle\pi,\C\rangle$.
(b) For discrete measures,
we can reformulate it as a linear problem
on a matrix whose rows sum up to the
weights of $\al$, and its columns to those of $\be$.
\\
In this paper, we focus on \emph{entropized}
transportation problems.
(c) The fuzziness induced by the \emph{positive}
regularization strength $\epsilon > 0$ turns
the sparse, combinatorial $\OT_0$-transport plan
into an analytic distribution.
Crucially, the $\OT_\epsilon$-transport plan (d)
can be encoded implicitly through the tensor sum
of two vectors $\b$ and $\a$, 
which are dual variables with respect
to $\alpha$ and $\beta$ --
see(\ref{eq-primal-dual}).
\label{fig:primal_problem}
}

\end{figure}




\paragraph{\emph{Relative} entropic regularization.}
Please note that we do not follow the conventions
of the reference paper ~\cite{CuturiSinkhorn},
in which the author implicitly makes use of the 
\emph{counting measure}
on the support of discrete distributions.
Instead, following~\cite{2016-genevay-nips}, we use a regularizer that is defined with respect to our source $\al$
and target $\be$:
this way, we are able to compare arbitrary
distributions (e.g. both discrete and continuous)
without inducing any bias through the choice of a reference
``counting'' measure.

Note, however, that our entropized problem still possesses
all the desirable properties of the usual
regularized OT costs.
First, in the limit case where $\epsilon=0$, 
we recover classical OT and 
$\OT_\epsilon \rightarrow \OT_0$ as 
$\epsilon \rightarrow 0$~\cite{leonard2012schrodinger,Carlier2017}. 
Furthermore, as discussed in the recent
handbook~\cite{peyre2017computational}
and in Section~\ref{sec:practice},
the transport cost $\OT_\epsilon(\al,\be)$
between two finitely supported measures
can be computed efficiently using the Sinkhorn iterations:
we have at hand a smooth and affordable loss function for
generic measure-fitting problems.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Dual ``Kantorovitch'' problem.}
The key to algorithmic efficiency comes
from the classical theory of \emph{convex duality}.
As we apply the Fenchel-Rockafellar theorem to
the $\OT_\epsilon$ problem,
we find a dual problem that reads
\begin{alignat*}{8}
\W_\epsilon(\al,\be)
\eqdef 
\max_{(\ab)\in \Cc(\Xx)^2}&
\langle\al,\f\rangle
+
\langle\be,\g\rangle \\
-\epsilon 
&\langle \al\otimes\be, 
e^{\big( \tfrac{1}{\epsilon}(\f\oplus \g - \C ) \big)} - 1 \rangle.
\nonumber %\\
%&=
%\max_{(f,g)\in\Cc(\Xx)^2}
%\int_\Xx f\d\al
%+ \int_\Xx g\d\be \\
%- \epsilon &\int_{\Xx^2}
%\exp\big(\tfrac{1}{\epsilon}(f(x)+g(y)-\C(x,y)) \big)
%\d\al(x)\d\be(y). \nonumber
\end{alignat*}
The primal-dual relationship linking an optimal primal 
$\pi$ solving~\eqref{eq-primal-ot} to an optimal
dual pair $(\ab)$ solving~\eqref{eq-dual} is
\begin{align*}
	\pi
	=
	\exp \big( \tfrac{1}{\epsilon} 
	(\f\oplus\g-\C) \big)\cdot(\al\otimes\be),
\end{align*}
and the optimality equations 
for the dual variables
(null derivatives in the dual problem), which are equivalent to the primal's marginal constraints on~\eqref{eq-primal-dual}, are
\begin{align}
\g(y)&= -\epsilon \log \int_\Xx \exp\big( \tfrac{1}{\epsilon}( 
	\f(x) - \C(x,y)
) \big) \d\al(x)\label{eq:dual_optimal_lse_a}\\
&\text{for $\be$-a.e. $y$, }\nonumber\\
\f(x)&= -\epsilon \log \int_\Xx \exp\big( \tfrac{1}{\epsilon}( 
	\g(y) - \C(x,y)
) \big) \d\beta(y)\label{eq:dual_optimal_lse_b}\\
&\text{for $\al$-a.e. $x$.}\nonumber
\end{align}
All-in-all, strong duality holds ~\cite{chizat2016scaling}: 
there exists a pair of 
continuous (and thus bounded) optimal potentials
$(\ab)$ for problem ~\eqref{eq-dual} such that
\begin{align}
\OT_\epsilon(\al,\be)=
\langle \al,\f\rangle
+ \langle \be,\g\rangle.\label{eq:strong_duality}
\end{align}



\paragraph{Naming the dual variables.}
Glancing at~\eqref{eq-dual}, our notations look surprising.
Why did we call ``$b$'' the Lagrange multiplier associated
to the $\alpha$-constraint and ``$a$'' the one associated
to $\be$?
Following the standard conventions of optimization theory
would also make sense: In the reference
handbook~\cite{peyre2017computational}, ``$b$''
is called ``$f$'' and ``$a$'' is called ``$g$''
so that~\eqref{eq:strong_duality} reads
\begin{align*}
\OT_\epsilon(\al,\be)=
\langle \al,f\rangle
+ \langle \be,g\rangle.
\end{align*}
Nevertheless, we argue that ``$b$ and $a$'' are
more suited than ``$f$ and $g$'' to a
\emph{geometric} understanding of Sinkhorn divergences.
Let us explain why.

In the next few pages, we show that the optimal dual potentials
are uniquely defined, up to an additive constant,
on the measures' supports~\eqref{eq:uniqueness_dual}.
In the meantime, such a pair of dual variables
can be canonically extended to the whole feature space $\Xx$
(\ref{eq:dual_optimal_X_a}-~\ref{eq:dual_optimal_X_b}) 
and displayed through contour lines
next to the samples of $\al$ and $\be$
-- see Figure~\ref{fig:dual_potentials}.

What appears, then, is that $a$ (resp. $b$) always behaves as a
\emph{shifted distance field} to the measure $\al$ (resp. $\be$).
This is made clear in the small and large $\epsilon$ limits
-- Proposition~\ref{prop:remarkable_potentials} --
and our main insight, detailed in~\cite{global-divergences}, is that the Sinkhorn
algorithm is all about \emph{balancing} distance fields
as it turns a Hausdorff distance into an OT cost.
$\OT_\epsilon(\al,\be)$ is, first and foremost,
a \emph{cross-correlation} term which interpolates between
$\OT_0(\al,\be)$ and $\langle \al,\C\star\be\rangle$.
By choosing letters that capture this coupling,
we are best able to stress the value of the
``unbiasing'' self-correlation terms in the
definition of the Sinkhorn
divergence $\Wb_\epsilon$ (\ref{eq-sinkhorn-div},~\ref{eq-sinkhorn-div}).

\paragraph{$\OT_\epsilon$ and Lipschitz functions.}

Let us remark that~\eqref{eq-dual}
can be rewritten as 
\begin{align*}
\OT_\epsilon(\al,\be)
=\max_{(\a,\b)\in\Cc(\Xx)^2}
&\langle\al,\b\rangle+\langle\be,\a\rangle\\
&-\langle\al\otimes\be,\iota_\epsilon(b\oplus a - \C)\rangle,
\end{align*}
where $\iota_\epsilon:x\mapsto \epsilon(\exp(x/\epsilon)-1)$
is a soft generalization of the indicator
function of the interval $(-\infty,0]$.
As $\epsilon$ tends to zero,
we thus retrieve the standard Kantorovitch problem:
\begin{align*}
\hspace{-.15cm}
\OT_0(\al,\be)&=
\max_{(\a,\b)\in\Cc(\Xx)^2}\langle\al,\b\rangle
+\langle\be,\a\rangle\\
&\text{s.t.} 
\forall x,y\in\Xx,
\b(x)+\a(y)\leqslant\C(x,y).
\end{align*}
If $\C(x,y)=\|x-y\|$, the true OT cost
$\OT_0(\al,\be)$ is then nothing but the dual norm
of $(\al-\be)$ with respect to the set
of $1$-Lipschitz functions.

This characterization of the Earth Mover's distance
has prompted recent interest in the machine learning
literature, as researchers strive to evaluate
OT-like divergences through Lipschitz
test functions encoded by convolutional neural 
networks~\cite{WassersteinGAN}.
From this perspective, our work should be understood
as a thorough study of the \emph{softening} 
of the Lipschitz constraint,
in the simple case where the cost function
$\C(x,y)$ between features is fully understood
-- i.e. when no neural net architecture is involved.
How useful these ideas can be to the GAN community
is still very much an open question.





\subsection{The SoftMin operator}
\label{sec:softmin}

\todo{Gab: I think this section can be removed.}


From an algorithmic perspective,
the identity~\eqref{eq:strong_duality} 
is a key result:
instead of computing the optimal transport cost $\OT_\epsilon(\al,\be)$
through a minimization on a variable $\pi$ or $p(x,y)$
that has a \emph{quadratic} memory footprint, 
we can simply work with a pair of functions $(\ab)$,
sampled on the supports of $\al$ and $\be$.

But we can go further.
In this work as in ~\cite{global-divergences}, we put 
a strong emphasis on the dual problem and the intuition
that can be built from it.
Instead of merely using it as a trick, a convenient proxy to
compute primal optimal transport costs~\cite{genevay2018learning,sharp_sinkhorn},
we now stress the geometric meaning 
of the equations(\ref{eq-dual}-\ref{eq:strong_duality}) and
reformulate them through the standard SoftMin
operator~\cite{peyre2017computational}.

\begin{defn}[SoftMin operator]
	Let $\epsilon > 0$ be a positive regularization strength.
Given a probability Radon measure $\al \in\Mm_1^+(\Xx)$
and a continuous function $\phi\in \Cc(\Xx)$
on the compact feature space $\Xx$,
we define the $\epsilon$-SoftMin of the values of $\phi$ on $\al$
through
\begin{align}
	\mine{x \sim \al} \phi(x) 
	\eqdef 
	-\epsilon\log \int_\Xx \exp\big(-\tfrac{1}{\epsilon} \phi(x)\big) \d\al(x).
\end{align}
\end{defn}

For a discrete measure $\al$, the SoftMin operator can be implemented efficiently and reliably on the GPU, as explained in Section~\ref{sec:practice}.
Moreover, it satisfies a few properties
that make it a convenient interpolator between
the simplest of all associative reduction operations: 
the \emph{minimum}
and the \emph{sum}, that correspond respectively
to the limit cases $\epsilon=0$ and $\epsilon=+\infty$.

\begin{prop}[The SoftMin interpolates between a minimum and a sum]
	Under the assumptions of the definition above, we get that
	\begin{align}
		\mine{x\sim \al} \phi(x) 
		&\xrightarrow{\epsilon\rightarrow 0} 
		\min_{ x \in \Supp(\al)} \phi(x) \\
		&\xrightarrow{\epsilon\rightarrow +\infty} 
		\qquad\langle\al,\phi\rangle.
	\end{align}
	If $\phi$ and $\psi$ are two continuous functions 
	in $\Cc(\Xx)$ such that $\phi \leqslant \psi$,
	\begin{align}
		\mine{x\sim \al} \phi(x) 
		\leqslant 
		\mine{x\sim \al} \psi(x). \label{eq:smin_order}
	\end{align}
	Finally, if $K\in\R$ is constant with respect to $x$, we have that 
	\begin{align}
		\mine{x\sim \al} \big[ K+\phi(x)\big]
		=&K+\mine{x\sim \al} \big[ \phi(x)\big].
		\label{eq:smin_constant}
	\end{align}
\end{prop}

\begin{prop}[The SoftMin operator is continuous]\label{prop:smin_continuous}
	Let $(\al_n)$ be a sequence of probability 
	measures converging \emph{weakly} towards $\al$,
	and $(\phi_n)$ be a sequence of continuous functions
	converging \emph{uniformly} towards $\phi$.
	Then, for $\epsilon>0$,
	the SoftMin of the values of $\phi_n$ on $\al_n$
	converges towards the SoftMin of the values of $\phi$
	on $\al$, i.e.
	\begin{align}
		\big( \al_n \rightharpoonup\al
		&,\,
		 \phi_n \xrightarrow{\|\cdot\|_\infty}\phi
		\big)\nonumber\\
		&\Longrightarrow
		\mine{x\sim \al_n} \phi_n(x)
		\rightarrow
		\mine{x\sim \al} \phi(x).
	\end{align}
\end{prop}

% 

\subsection{Dual potentials}


\paragraph{Fixed point equation.}
Using the SoftMin operator,
we can rewrite the optimality equations
(\ref{eq:dual_optimal_lse_a}-~\ref{eq:dual_optimal_lse_b})
in a meaningful way:
\begin{align*}
	\g(y)&= \mine{x\sim\al}\big[ \C(x,y)-\f(x) \big]
	&&\text{for $\be$-a.e. $y$,}\\
	\f(x)&= \mine{y\sim\be}\big[ \C(x,y)-\g(y) \big]
	&&\text{for $\al$-a.e. $x$.}
\end{align*}
If we introduce the ``Sinkhorn mapping'' $\T: \Mm_1^+(\Xx)\times\Cc(\Xx) \rightarrow \Cc(\Xx)$ in the log-domain, 
\begin{align}
	\hspace{-.3cm}
	\T : (\al,\f) \mapsto \bigg( y\in\Xx \mapsto 
	\mine{x\sim\al} \big[ 
	 \C(x,y) -\f(x)	
	\big]
	\bigg),
\end{align}
we see that $(\ab)$ is an optimal dual pair if and only if
\begin{align}
	& \g&= \T(\al,\f)\; \text{$\be$-a.e.}
	&\text{and}&
	\f&= \T(\be,\g)\;\text{$\al$-a.e.}
\end{align}
The Sinkhorn algorithm, detailed in section~\ref{sec:practice},
is all about alternatively enforcing these two conditions
on the pair $(\ab)$.

\paragraph{Dual potentials on the feature space.}

Now, remark that as far as algorithms and cost values are concerned,
$\g$ and $\f$ only need to be defined on the supports of $\be$ and $\al$,
respectively.
Equations(\ref{eq:dual_optimal_smin_a}-\ref{eq:dual_optimal_smin_b}),
however, allow us to \emph{extend} optimal potentials
to the whole feature space in a canonical way.
Just as in the classical theory of OT~\cite[Remark 1.13]{santambrogio2015optimal},
we will now assume that every pair of optimal dual potentials 
satisfies these equations \emph{for all $x$ and $y$}:
\begin{align}
	\foralls y\in\Xx, \g(y)
	&= \mine{x\sim\al}\big[ \C(x,y)-\f(x) \big],
	\label{eq:dual_optimal_X_a}\\
	\foralls x \in \Xx, \f(x)
	&= \mine{y\sim\be}\big[ \C(x,y)-\g(y) \big].
	\label{eq:dual_optimal_X_b}
\end{align}


%\begin{rem}[On the dual potentials] \label{rem-definition} %Even though the definition of the potentials only matter on the support of $(\al,\be)$, one can define them on $\Xx$ by iterating the Sinkhorn mapping one last time $\forall \; x\in\Xx$. Those mapping can be defined outside of the measures' supports and it maintains the fixed-point property on $\Xx$. In what follows, it is in that sense that we define the optimal potentials on $\Xx$.
%The value of the dual potentials only matter on the support of the reference measures. We know that on their support the dual potentials are obtained via a Soft-c-Transform which is a regularization of the concept of c-convex functions. Similar to classical OT (see~\cite{santambrogio2015optimal}), the solution on the whole domain $\Xx$ is not unique in $\Cc(\Xx)$, but we have unicity of the "Soft-c-concave" solution. In other terms, we can extend our optimal potentials defined on the support of $(\al,\be)$ via the transformations $(T,S)$ mentioned above which defines "Soft-c-concave" functions on $\Xx$. In what follows, when considering the optimal dual potentials defined on $\Xx$ we will use this extended solution.
%\end{rem}

\paragraph{First properties.}
Optimal dual potentials satisfy a host of convenient
properties, that we now present.
Please note that, as advertised in section~\ref{sec:assumptions},
these results hold
under the assumption that $(\Xx,\d)$ is a compact metric space,
endowed with a \emph{ground cost} function $\C:\Xx\times\Xx\rightarrow\R$
that is $\kappa$-Lipschitz with respect to both of its input variables.

\begin{prop}[Lipschitz property]
The optimal potentials $(\ab)$ of the dual problem(\ref{eq-dual})
are both $\kappa$-Lipschitz functions on the feature space $(\Xx,\d)$.
\end{prop}
\begin{proof}
According to ~\eqref{eq:dual_optimal_X_a}, 
$\g$ is a SoftMin combination of 
$\kappa$-Lipschitz functions of the variable $y$;
using the algebraic properties of the SoftMin operator
detailed in (\ref{eq:smin_order}-~\ref{eq:smin_constant}), 
one can thus show that $\g$ is a $\kappa$-Lipschitz function
on the feature space.
The same argument holds for $\f$.
\end{proof}

% \paragraph{Link between MMD and OT.}



\begin{figure}[t!]
  \centering

	\begin{subfigure}[t]{.6\linewidth}
		\centering
		\includegraphics[width=\linewidth]{sections/images/sinkhorn_L1_S_100its.png}
		\caption{$p=1$, $\epsilon=\texttt{.01}$.}
	\end{subfigure}
	
	\begin{subfigure}[t]{.6\linewidth}
		\centering
		\includegraphics[width=\linewidth]{sections/images/sinkhorn_L1_L_100its.png}
		\caption{$p=1$, $\epsilon=\texttt{.10}$.}
	\end{subfigure}
	
	\begin{subfigure}[t]{.6\linewidth}
		\centering
		\includegraphics[width=\linewidth]{sections/images/sinkhorn_L2_L_100its.png}
		\caption{$p=2$, $\sqrt{\epsilon}=\texttt{.10}$.}
	\end{subfigure}
  
  \caption{
    \textbf{Displaying the optimal dual potentials.}
    The discrete measures $\al$ and $\be$
    are displayed through their red and blue samples
    in the unit square.
    In the background, we display the optimal pair
    $(a,b)$ of dual potentials for $\OT_\epsilon(\al,\be)$,
    using a ground cost $\C(x,y)=\|x-y\|^p$ and a regularization
    strength $\epsilon>0$:
    the contour lines of $a$ are drawn in red,
    those of $b$ in blue.
    \label{fig:dual_potentials}}
\end{figure}


The following proposition is a continuous analogous, in the log-domain, of the celebrated result of Sink\-horn~\cite{Sinkhorn64}
on the uniqueness up to a multiplicative constant of scaling coefficients for positive matrices.
Combined with (\ref{eq:dual_optimal_X_a}-~\ref{eq:dual_optimal_X_b}), 
it allows us to
\emph{display} the optimal pair of dual potentials for any given
pair of probability measures -- see Figure~\ref{fig:dual_potentials}.

\begin{prop}[Uniqueness of the dual potentials up to an additive constant] 
	\label{prop:uniqueness_dual}
Let $(\g_0,\f_0)$ and $(\g_1,\f_1)$ be two optimal pairs
of dual potentials for a problem $\W_\epsilon(\al,\be)$
that satisfy (\ref{eq:dual_optimal_X_a}-~\ref{eq:dual_optimal_X_b}).
Then, there exists a constant $K\in\R$ such that
\begin{align}
	\g_0 = \g_1 - K~\text{and}~\f_0= \f_1+K.
	\label{eq:uniqueness_dual}
\end{align}
\end{prop}
\begin{proof}
	For $t\in[0,1]$, let us define
	$\g_t = \g_0 + t(\g_1-\g_0)$,
	$\f_t = \f_0 + t(\f_1-\f_0)$ and
	\begin{align*}
	\phi(t)= 
	&\langle\al,\f_t\rangle
	+
	\langle\be,\g_t\rangle\\
	&-
	\epsilon\langle\al\otimes\be,
	\exp\big(\tfrac{1}{\epsilon}(\f_t\oplus \g_t - \C)\big)-1\rangle,
	\end{align*}
	the value of the dual objective between the two optimal pairs.
	As $\phi$ is a concave function bounded above by 
	$\phi(0)=\phi(1)=\W_\epsilon(\al,\be)$, it is \emph{constant} with respect to $t$.
	Hence, for all $t$ in $[0,1]$,
	\begin{align*}
		\hspace{-.3cm}
		0 &= \phi''(t)\\
		&=
		-\tfrac{1}{\epsilon}
		\langle \al\otimes\be,
		e^{\big( \tfrac{1}{\epsilon}(\f_t\oplus \g_t - \C) \big)}
		((\f_1-\f_0)\oplus (\g_1-\g_0))^2\rangle.
	\end{align*}
	This is only possible if 
	\begin{align*}
		\big(\f_1(x)-\f_0(x)+\g_1(y)&-\g_0(y)\big)^2=0 \\&\text{$\al\otimes\be$-a.e. in $(x,y)$},
	\end{align*}
	i.e. there exists a constant $K\in\R$ such that
	\begin{align*}
		&\g_1(y)-\g_0(y)=-K\quad\text{$\be$-a.e.}\\
		& \f_1(x)-\f_0(x)= +K\quad\text{$\al$-a.e.}
	\end{align*}
	As we extend the potentials through 
	(\ref{eq:dual_optimal_X_a}-\ref{eq:dual_optimal_X_b}), 
	the SoftMin operator commutes with the addition of $K$
	and lets our result hold on the whole feature space.
\end{proof}


\todo{Gab: I think this proposition can be removed.}

\begin{prop}[Remarkable values of $\W_\epsilon$ and its dual potentials]
  \label{prop:remarkable_potentials}
  Let $\al$ and $\be$ be two
  probability Radon measures in $\Mm_1^+(\Xx)$,
  and for $\epsilon > 0$, let us denote
  by $(\g_\epsilon,\f_\epsilon)$ a pair
  of optimal dual potentials for $\W_\epsilon(\al,\be)$
  -- which are uniquely defined up to an additive constant
  (Prop.~\ref{prop:uniqueness_dual}).
  Then, the following holds:
  \begin{enumerate}
  
  \item If $\al = \delta_{x_o}$ and $\be=\delta_{y_o}$
  are two Dirac measures, then for all $z\in\Xx$,
  \begin{align}
  \g_\epsilon(z)&= \C(x_o,z), \quad
  \f_\epsilon(z)= \C(z,y_o)-\C(x_o,y_o), \nonumber \\
  \text{i.e.}
  \g_\epsilon&= \C\star\al,\quad
  \f_\epsilon= \C\star\be-\C(x_o,y_o).
  \label{eq:dual_diracs}
  \end{align}
  This implies that for all $\epsilon$,
  $\W_\epsilon(\delta_{x_o}, \delta_{y_o})=\C(x_o,y_o)$.
  
  \item For any $\al$ and $\be$, as $\epsilon\rightarrow\infty$, we have
  \begin{align}
  \g_\epsilon\xrightarrow{\|\cdot\|_\infty} \C\star\al,
  \qquad
  \f_\epsilon\xrightarrow{\|\cdot\|_\infty} \C\star\be-\langle \al, \C\star\be\rangle.
  \label{eq:dual_infinity}
  \end{align}
  Combining this with ~\eqref{eq:strong_duality}, we get
  \begin{align*}
   \W_\epsilon(\al, \be)
  \xrightarrow{\epsilon\rightarrow+\infty}
  \langle \al, \C\star\be\rangle.
  \end{align*}
  \end{enumerate}
\end{prop}

\begin{proof}
\emph{Proof of 1.}
The optimality conditions
(\ref{eq:dual_optimal_X_a}-~\ref{eq:dual_optimal_X_b}) read
\begin{alignat*}{8}
\foralls y\in\Xx, \g_\epsilon(y)
	&= \mine{x\sim\delta_{x_o}}\big[ \C(x,y)-\f(x) \big]\\
	&=
	\C(x_o,y) - \f_\epsilon(x_o), \\
	\foralls x \in \Xx, \f_\epsilon(x)
	&= \mine{y\sim\delta_{y_o}}\big[ \C(x,y)-\g(y) \big]\\
	&=
	\C(x,y_o) - \g_\epsilon(y_o),
\end{alignat*}
and are satisfied by the potentials defined in ~\eqref{eq:dual_diracs}.
We then have
\begin{alignat*}{8}
\W_\epsilon(\delta_{x_o},\delta_{y_o})&=
\langle\delta_{x_o},\f_\epsilon\rangle
&+&
\langle\delta_{y_o},\g_\epsilon\rangle\\
&= \C(x_o,y_o) - \C(x_o,y_o) &+&
\C(x_o,y_o).
\end{alignat*}

\noindent \emph{Proof of 2.}
Let us disambiguate the choice of $(\g_\epsilon,\f_\epsilon)$
by assuming that $\langle\al,\f_\epsilon\rangle=0$ for
all $\epsilon$.
Since $(\f_\epsilon,\g_\epsilon)$ are both $\kappa$-Lipschitz
functions on the bounded, compact set $\Xx$, we can then produce
uniform bounds on $\f_\epsilon$ and $\g_\epsilon$
-- using ~\eqref{eq:dual_optimal_X_a} -- that hold
for any $\epsilon>0$ and point on the feature space.

Using a Taylor expansion of $\exp$ in the optimality
equations (\ref{eq:dual_optimal_lse_a}-\ref{eq:dual_optimal_lse_b}),
we get 
\begin{alignat*}{8}
\g_\epsilon&=\C\star\al
&-&\langle\al,\f_\epsilon\rangle
&+& \tfrac{1}{\epsilon}e_{1,\epsilon} \\
\f_\epsilon&=\C\star\be
&-&\langle\be,\g_\epsilon\rangle
&+& \tfrac{1}{\epsilon}e_{2,\epsilon},
\end{alignat*}
where $e_{1,\epsilon}$ and $e_{2,\epsilon}$
are uniformly bounded residuals.
Since $\langle\al,\f_\epsilon\rangle=0$ and $\C$ is 
a symmetric cost function,
we have ~\eqref{eq:dual_infinity}.
Finally, keeping in mind that
$\al$ is a probability measure, i.e.
$\langle\al,1\rangle=1$, we get
\begin{align*}
\W_\epsilon(\al,\be) &=
\langle\al,\f_\epsilon\rangle
+
\langle\be,\g_\epsilon\rangle \\
&\xrightarrow{\epsilon\rightarrow+\infty}
\langle \al,\C\star\be\rangle - 
\langle\al,1\rangle
\langle \al,\C\star\be\rangle\\
&\qquad\qquad+
\langle \al,\C\star\be\rangle.
\end{align*}
\end{proof}

\subsection{Gradients of the regularized OT cost}


\paragraph{Regularity of $\OT_\epsilon$.}
In the previous section, we have seen that 
the optimal dual potentials $\g$ and $\f$
for ~\eqref{eq-dual} are \emph{continuous}
functions on the feature space,
\emph{uniquely} defined up to an additive constant.
We now show that they are no one but the
\emph{gradients} of $\W_\epsilon(\al,\be)$, in the sense
of~(\ref{eq:dual_optimal_X_a},~\ref{eq:dual_optimal_X_b}).


Please note that another proof of this result
is possible, by relying on the 
fact that the Sinkhorn mapping is
a contraction with respect to the Hilbert projective 
metric~\cite{lemmens2012nonlinear}.
After a few pages of technical derivations, 
using the implicit function theorem,
it is possible
to show that the optimal potentials vary in a
locally Lipschitz way along variations of the input measures.
Then, we can simply use the null value of the 
dual objective's derivatives at the optimum to show
that Corollary~\ref{thm-differentiability} holds.


\begin{lem}[The dual potentials vary continuously with the input measures] 
\label{lem-uniform-conv}
Let $\al_n \rightharpoonup \al$ and 
$\be_n \rightharpoonup \be$ be weakly converging 
sequences of measures in $\Mm_1^+(\Xx)$.
Given some arbitrary anchor point $x_o\in\Xx$,
let us denote by $(\g_n,\f_n)$ the (unique) sequence of optimal
potentials for $\W_\epsilon(\al_n,\be_n)$ such that $\g_n(x_o)=0$.

Then, $\g_n$ and $\f_n$ converge uniformly towards the 
unique pair of optimal potentials $(\ab)$ for $\W_\epsilon(\al,\be)$
such that $\g(x_o)=0$.
Up to the value at the anchor point $x_o$, we thus have that
\begin{align*}
\big( \al_n \rightharpoonup \al, \,
\be_n \rightharpoonup \be
\big)\Longrightarrow
\big( \g_n \xrightarrow{\|\cdot\|_\infty} \g, \,
\f_n \xrightarrow{\|\cdot\|_\infty} \f
\big).
\end{align*}
\end{lem}
\begin{proof}
	For all $n$ in $\mathbb{N}$, the potentials $\g_n$ and $\f_n$
	are $\kappa$-Lipschitz functions on the compact, bounded set $\Xx$.
	As $\g_n(x_o)$ is set to zero, we can bound $|\g_n|$ on $\Xx$
	by $\kappa$ times the diameter of $\Xx$;
	combining this with (\ref{eq:dual_optimal_X_b}),
	we can then produce a uniform bound on both $\g_n$ and $\f_n$:
	there exists a constant $M\in\R$ such that 
	\begin{align*}
		\foralls n\in\mathbb{N}, \foralls x\in\Xx, 
		-M\leqslant \g_n(x), \f_n(x) \leqslant+M.
	\end{align*}
	
	Being equicontinuous and uniformly bounded on the compact set $\Xx$,
	the sequence $(\g_n,\f_n)_n$ satisfies the hypotheses of the
	Ascoli-Arzelà theorem: there exists a subsequence $(\g_{n_k},\f_{n_k})_k$
	that converges uniformly towards a pair $(\ab)$ of continuous functions.
	Letting $k$ tend to infinity, we see that $\g(x_o)=0$ and,
	using the continuity of the SoftMin operator (Proposition~\ref{prop:smin_continuous})
	on the optimality equations(\ref{eq:dual_optimal_X_a}-~\ref{eq:dual_optimal_X_b}),
	we show that $(\ab)$ is an optimal pair for $\W_\epsilon(\al,\be)$.

	Now, according to Proposition~\ref{prop:uniqueness_dual},
	such a limit pair of optimal potentials $(\ab)$ is \emph{unique}.
	$(\g_n,\f_n)_n$ is thus a \emph{compact} sequence with a 
	\emph{single} possible adherence value:
	it has to converge, uniformly, towards $(\ab)$.
\end{proof}


\begin{cor}[The regularized OT cost is weakly continuous]
	\label{thm-continuity}
	Assuming that $(\Xx,\d)$ is a compact metric space endowed
	with a Lipschitz cost function $\C$,
	\begin{align*}
		\W_\epsilon : (\al,\be)\in \Mm_1^+(\Xx)^2
		\mapsto \W_\epsilon(\al,\be)\in \R
	\end{align*}
	is continuous with respect to the convergence in law.
\end{cor}

\begin{proof}
	As written in ~\eqref{eq:strong_duality}, 
	$\W_\epsilon(\al,\be)$ can be computed through a straightforward,
	\emph{continuous} expression that does not depend
	on the value of the optimal dual potentials $(\ab)$
	at the anchor point $x_o$:
	\begin{align*}
		\W_\epsilon(\al,\be)=
		\langle\al,\f\rangle+
		\langle\be,\g\rangle.
	\end{align*}
	Combining this equation with Lemma~\ref{lem-uniform-conv}
	(that guarantees the \emph{uniform} convergence of potentials 
	for weakly converging sequences of probability measures)
	allows us to conclude.
\end{proof}

\begin{cor}[The dual potentials are the gradients of the regularized OT cost]
	\label{thm-differentiability}
	Under the same assumptions,
	$\W_\epsilon$ is a differentiable function on
	$\Mm_1^+(\Xx)\times\Mm_1^+(\Xx)$ -- in the sense
	of~(\ref{eq:dual_optimal_X_a},~\ref{eq:dual_optimal_X_b}).
	If $(\ab)$ is a pair of optimal potentials for $(\al,\be)$,
	uniquely defined up to an additive constant, we have
	\begin{align}
  \nabla \W_\epsilon (\al,\be)
  =(\f,\g),
  \label{eq:gradient_ote}
  \end{align}
  which should not be confused with $(a,b)$.
  That is, for any admissible variations
  $\delta\al$ and $\delta\be$ in $\Mm_0(\Xx)$
  and time $t$ in a neighborhood of $0$ such that
  $\al + t\delta\al$ and $\be+t\delta\be$
  both belong to $\Mm_1^+(\Xx)$, we have
  \begin{align*}
  \W_\epsilon(\al + t\delta\al, \be+t\delta\be)
  &= \W_\epsilon(\al,\be)\\
  &+
  t\big(\langle \delta\al,\f\rangle
  +\langle\delta\be,\g\rangle\big)+o(t).
  \end{align*}
  Note that since
  $\langle\delta\al,1\rangle=\langle\delta\be,1\rangle=0$,
  these gradients are only defined up to an additive constant.
\end{cor}

\begin{proof}
The proof is mainly inspired 
from~\cite[Proposition 7.17]{santambrogio2015optimal}. 
Let us consider $\al$, $\delta\al$, $\be$, $\delta\be$
and times $t$ in a neighborhood of $0$, as in the statement above.
We define $\al_t=\al+t\delta\al$,
$\be_t=\be+t\delta\be$ and the variation ratio $\De_t$
given by
\begin{align*}
\De_t \eqdef \frac{\W_\epsilon(\al_t,\be_t) - \W_\epsilon(\al,\be)}{t}.
\end{align*}
Using the very definition of $\W_\epsilon$
and the continuity Lemma~\ref{lem-uniform-conv},
we now provide lower and upper bounds on $\De_t$
as $t$ goes to $0$.

\noindent
\emph{Lower bound.}
First, let us remark that $(\ab)$ is a
\emph{suboptimal} pair of dual potentials for
$\W_\epsilon(\al_t,\be_t)$.
Hence,
\begin{align*}
\W_\epsilon(\al_t,\be_t)
&\geqslant
\langle\al_t,\f\rangle
+
\langle\be_t,\g\rangle \\
&-
\epsilon\langle \al_t\otimes\be_t
, \exp\big( \tfrac{1}{\epsilon}( \f\otimes \g - \C) \big)-1\rangle
\nonumber
\end{align*}
and thus, since 
\begin{align*}
 \W_\epsilon(\al,\be) &= \langle\al,\f\rangle
+\langle\be,\g\rangle\\
&-\epsilon \langle\al\otimes\be, \exp(\tfrac{1}{\epsilon}(\f\oplus \g-\C))-1\rangle,
\end{align*}
\begin{align*}
\De_t &\geqslant
\langle\delta\al,\f\rangle
+
\langle\delta\be,\g\rangle\\
&- \epsilon 
\langle \delta\al\otimes\be +
\al\otimes\delta\be , \exp(\tfrac{1}{\epsilon}(\f\oplus \g-\C))
\rangle+o(1) \nonumber \\
&\geqslant
\langle\delta\al,\f-\epsilon\rangle
+
\langle\delta\be,\g-\epsilon\rangle+o(1),
\end{align*}
since $\g$ and $\f$ satisfy the optimality 
equations (\ref{eq:dual_optimal_lse_a}-\ref{eq:dual_optimal_lse_b}).

\noindent
\emph{Upper bound.}
Conversely, let us denote by $(\g_t,\f_t)$ the optimal pair 
of potentials for $\W_\epsilon(\al_t,\be_t)$
satisfying $\g_t(x_o)=0$ for some arbitrary
anchor point $x_o\in\Xx$.
As $(\g_t,\f_t)$ are suboptimal potentials for $\W_\epsilon(\al,\be)$,
we get that
\begin{align*}
\W_\epsilon(\al,\be)
&\geqslant
\langle\al ,\f_t\rangle
+
\langle\be,\g_t\rangle \\
&-
\epsilon\langle \al\otimes\be
, \exp\big( \tfrac{1}{\epsilon}( \f_t\otimes \g_t - \C) \big)-1\rangle
\nonumber
\end{align*}
and thus, since 
\begin{align*}
 \W_\epsilon(\al_t,\be_t) &= \langle\al_t,\f_t\rangle+\langle\be_t,\g_t\rangle\\
 &-\epsilon \langle\al_t\otimes\be_t, \exp(\tfrac{1}{\epsilon}(\f_t\oplus \g_t-\C))-1\rangle,
\end{align*}
\begin{align*}
\De_t &\leqslant
\langle\delta\al,\f_t\rangle
+
\langle\delta\be,\g_t\rangle\\
&- \epsilon 
\langle \delta\al\otimes\be_t +
\al_t\otimes\delta\be 
, \exp(\tfrac{1}{\epsilon}(\f_t\oplus \g_t-\C))
\rangle+o(1) \nonumber \\
&\leqslant
\langle\delta\al,\f_t-\epsilon\rangle
+
\langle\delta\be,\g_t-\epsilon\rangle+o(1).
\end{align*}

\noindent
\emph{Conclusion.}
Now, let us remark that as $t$ goes to $0$
\begin{align*}
\al+t\delta\al &\rightharpoonup \al
& \text{and}&
&
\be+t\delta\be &\rightharpoonup \be.
\end{align*}
Thanks to Lemma~\ref{lem-uniform-conv},
we thus know that $\g_t$ and $\f_t$ converge uniformly
towards $\g$ and $\f$.
Combining the lower and upper bound, we get
\begin{align*}
\De_t \xrightarrow{t\rightarrow0}
\langle\delta\al,\f-\epsilon\rangle
+
\langle\delta\be,\g-\epsilon\rangle
=
\langle\delta\al,\f\rangle
+
\langle\delta\be,\g\rangle,
\end{align*}
since $\delta\al$ and $\delta\be$ both have
an overall mass that sums up to zero.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proofs of main properties}

In this section we recall some of the results presented in the main corpus whose proof has been sketched rather than rigorously proved.

\begin{prop}[The Sinkhorn negentropy is an entropized kernel norm]
For $\epsilon > 0$ and $\al\in\Mm_1^+(\Xx)$, we have
\begin{alignat}{8}
	\tfrac{1}{\epsilon}\,\F_\epsilon(\al)
	+\tfrac{1}{2}&=
& &\min_{\mu\in\Mm^+(\Xx)}
&\langle \al, \log \tfrac{\d \al}{\d \mu} \rangle
&+\tfrac{1}{2} \|\mu\|_{k_\epsilon}^2
&&\\
&=& &\min_{\mu\gg\al}
&\langle \al, \log \tfrac{\d \al}{\d \mu} \rangle
&+ \tfrac{1}{2} \langle \mu,
k_\epsilon\star \mu\rangle \nonumber
&&. 
\end{alignat}
\end{prop}

\begin{proof}
The definition of $\W_\epsilon(\al,\al)$ is that
\begin{align*}
\W_\epsilon(\al,\al)
=
\max_{(\ab)\in \Cc(\Xx)^2}
&\langle\al,\f+\g\rangle\\
&-\epsilon
\langle \al\otimes\al,
e^{\big( \tfrac{1}{\epsilon}(\f\oplus \g - \C ) \big)}-1 \rangle.
\end{align*}


\noindent
\emph{Reduction of the problem.}
Thanks to the symmetry of this concave problem
with respect to the variables $\g$ and $\f$,
we know that there exists a pair $(\g,\f=\g)$
of optimal potentials on the diagonal, and
\begin{alignat*}{8}
\W_\epsilon(\al,\al)
=
&\max_{\g\in \Cc(\Xx)}
2 \langle\al,\g\rangle\\
&\quad -\epsilon 
\langle \al\otimes\al,
e^{\big( \tfrac{1}{\epsilon}(\g\oplus \g - \C ) \big)}-1 \rangle \\
= 
&\max_{\g\in \Cc(\Xx)}
 2 \langle\al,\g\rangle\\
&\quad -\epsilon
\langle \exp(\g/\epsilon)\al, 
k_\epsilon\star \exp(\g/\epsilon)\al\rangle
+\epsilon.
\end{alignat*}

\noindent
\emph{Change of variables.}
Let us remark that this maximimization
can be made on the full set of $\alpha$-measurable
functions: through the optimality equations,
one can check that a solution of this extended problem
would necessarily be continuous on $\Xx$.
Through a change of variables
\begin{align*}
\mu&=\exp(\g/\epsilon)\al
&\text{i.e.}& &
\g&= \epsilon\log\tfrac{\d\mu}{\d\al},
\end{align*}
keeping in mind that
$\al$ is a probability measure,
we thus get that
\begin{alignat*}{8}
\W_\epsilon(\al,\al)
=
\epsilon\max_{\mu\in\Mm^+(\Xx),\al\ll\mu\ll\al}
&2 \langle\al,\log \tfrac{\d\mu}{\d\al}\rangle
\\- 
&\langle \mu, 
k_\epsilon\star \mu \rangle
+1\\
-\tfrac{1}{2}\W_\epsilon(\al,\al)
=
\epsilon\min_{\mu\in\Mm^+(\Xx),\al\ll\mu\ll\al}
&\langle\al,\log \tfrac{\d\al}{\d\mu}\rangle
\\ +\tfrac{1}{2}
&\langle \mu,
k_\epsilon\star \mu \rangle
-\tfrac{1}{2},
\end{alignat*}
where we optimize on measures $\mu \in\Mm^+(\Xx)$
such that $\al \ll \mu$ \text{and} $\mu \ll \al$.

~\\
\noindent
\emph{Expansion of the problem.}
As $k_\epsilon(x,y)=\exp(-\C(x,y)/\epsilon)$ 
is positive for all $x$ and $y$ in $\Xx$,
we can remove the $\mu\ll\al$ constraint from the optimization problem:
\begin{alignat*}{8}-\tfrac{1}{2}\W_\epsilon(\al,\al)=
\epsilon\min_{\mu\in\Mm^+(\Xx),\al\ll\mu}
&\langle\al,\log \tfrac{\d\al}{\d\mu}\rangle
\\+\tfrac{1}{2}
&\langle \mu, 
k_\epsilon\star \mu \rangle
-\tfrac{1}{2}.
\end{alignat*}
Indeed, restricting a positive measure $\mu$ 
to the support of $\al$ lowers the right-hand term
without having any influence on the density 
of $\al$ with respect to $\mu$.
Finally, let us remark that the $\al\ll\mu$ constraint
is already encoded in the $\log\tfrac{\d\al}{\d\mu}$ operator,
which blows up to infinity if $\al$ has no density with respect to $\mu$;
all in all, we thus have:
\begin{alignat*}{8}
\F_\epsilon(\al)
&=-\tfrac{1}{2}\W_\epsilon(\al,\al)\\
&=
\epsilon\min_{\mu\in\Mm^+(\Xx)}
\langle\al,\log \tfrac{\d\al}{\d\mu}\rangle
+\tfrac{1}{2}
\langle \mu, 
k_\epsilon\star \mu \rangle-\tfrac{1}{2}
,
\end{alignat*}
which is the desired result.
\end{proof}

\begin{thm}[Strict convexity of the Sinkhorn negentropy]
  Let $(\Xx,\d)$ be a compact set endowed with a symmetric,
  Lipschitz cost function $\C(x,y)$ that induces
  a \emph{positive} kernel $k_\epsilon$:
  Then, $\F_\epsilon$ is a \emph{strictly convex} functional
  on $\Mm_1^+(\Xx)$.
\end{thm}
\begin{proof}
The relative entropy
$(\al,\mu)\mapsto\langle\al,\log\tfrac{\d\al}{\d\mu}\rangle$
is a jointly convex function -- as a pointwise
perspective transform of minus $\log$.
Since $k_\epsilon$ is assumed to define a
\emph{positive} kernel function,
\begin{align*}
\E_\epsilon:(\al,\mu)
\mapsto
\epsilon\langle \al, \log \tfrac{\d \al}{\d \mu} \rangle
+\tfrac{\epsilon}{2} \|\mu\|_{k_\epsilon}^2
-\tfrac{\epsilon}{2}
\end{align*}
is thus (jointly) strictly convex.

Being defined as its marginalization on a convex set,
$\F_\epsilon$ is then strictly convex
too. Indeed, we know from OT theory that the solution $\mu$ always exists and is attained, thus we show the strict convexity by applying inequalities to $\F_\epsilon$ which equals $\E_\epsilon$ at the optimum and is strictly convex. 
% Let us take $\al_0\neq\al_1$ a pair of measures
% $\Mm_1^+(\Xx)$,
% and $t\in(0,1)$;
% according to ~\eqref{eq-sinkh-entropy},
% there exists a pair of measures $\mu_0$, $\mu_1$ 
% in $\Mm^+(\Xx)$ such that
% \begin{align*}
% (1-t)&\F_\epsilon(\al_0)
% + t\F_\epsilon(\al_1)\\
% &=
% (1-t)\E_\epsilon(\al_0,\mu_0)
% +t\E_\epsilon(\al_1,\mu_1) \\
% &>
% \E_\epsilon((1-t)\al_0 + t\al_1, (1-t)\mu_0 + t\mu_1) \\
% &\geqslant
% \F_\epsilon((1-t)\al_0 + t\al_1),
% \end{align*}
% which is enough to conclude.
%Lastly, we need to justify the strict concavity of the functional $\Hh_\epsilon$. First, $\KL(\cdot|\cdot)$ is strictly convex since it is a f-divergence, and strict convexity is preserved by perspective transformations. Second, $\Hh_\epsilon$ is concave as a maximization of concave functions over a convex set. The strict concavity can be shown by mentioning that in equation~\eqref{eq-sinkh-entropy} the optimal potential exists and is attained in $\Cc(\Xx)$, thus the optimal measure is also attained in~\eqref{eq-fundamental}. Such property allows to show that we preserve strict concavity.
%Since $\KL(\cdot|\cdot)$ is jointly convex of both its arguments, $\Hh_\epsilon$ is the marginalization of a jointly (strictly) concave function (see~\cite[Corollary 2.9]{liero2015optimal}) and is hence strictly concave. 
\end{proof}

\begin{thm}[The Hausdorff and Sinkhorn divergences
metrize the convergence in law]
Under the same assumptions as Theorem~\ref{thm-global-positivity},
$\H_\epsilon$ and
$\Wb_\epsilon$ metrize the convergence in law, i.e for any sequence $\al_n$ in
$\Mm_1^+(\Xx)$, we have
\begin{align*}
\H_\epsilon(\al_n,\al)
\rightarrow 0
\Longleftrightarrow
\al_n\rightharpoonup\al
\Longleftrightarrow
\Wb_\epsilon(\al_n,\al)
\rightarrow 0.
\end{align*}
\end{thm}

\begin{proof}
The regularized OT cost is weakly continuous, and the uniform convergence
for dual potentials
ensures that $\H_\epsilon$ and
$\Wb_\epsilon$ are both continuous.
Paired with ~\eqref{eq:divergence_definite},
this property guarantees
the convergence towards $0$ of the Hausdorff and Sinkhorn divergences,
as soon as $\al_n \rightharpoonup\al$.

Conversely, let us assume that $\Wb_\epsilon(\al_n,\al)\rightarrow 0$ (resp. $\H_\epsilon(\al_n,\al)$).
Any weak limit $\al_{n_\infty}$
of a subsequence $(\al_{n_k})_k$ is equal to $\al$:
since our divergence is weakly continuous,
we have $\Wb_\epsilon(\al_{n_\infty},\al)=0$
(resp. $\H_\epsilon(\al_{n_\infty},\al)$),
and positive definiteness holds through ~\eqref{eq:divergence_definite}.

In the meantime, since $\Xx$ is compact, 
the set of probability Radon measures $\Mm_1^+(\Xx)$ is 
sequentially compact for the weak-$\star$
topology.
$\al_n$ is thus a compact sequence with a unique adherence
value: it converges, towards $\al$.
%Since we assume all measures to be compact on $\Xx$ compact, we can extract a converging subsequence $\al_{n_k} \rightharpoonup \nu$. Since $\bar \W_\epsilon$ is continuous (as a consequence of Theorem~\ref{thm-continuity}) we get that $\bar{W}_\epsilon(\nu,\al)=0 \; \Rightarrow \; \nu = \al$. Thus, we get that necessarily $\al_n \rightharpoonup \al$.
\end{proof}


\todo{Gab: I think this proposition can be removed.}

\begin{prop}[The Sinkhorn divergence interpolates between
  an OT loss and an MMD]
	For $\al$ and $\be$ in $\Mm_1^+(\Xx)$, we have
	\begin{alignat}{8}
		\Wb_\epsilon(\al,\be) 
		&\xrightarrow{\epsilon \rightarrow ~0}
		\OT_0(\al,\be) - \tfrac{1}{2}\OT_0(\al,\al)
		- \tfrac{1}{2}\OT_0(\be,\be)\\
		&\xrightarrow{~\epsilon\rightarrow +\infty}
		\tfrac{1}{2}\norm{\al-\be}_{-\C}^2.
	\end{alignat}
	Note that for all standard cost functions,
	$\C(x,y) \geqslant 0$ with equality iff. $x=y$
	so that $\OT_0(\al,\al) = 0 = \OT_0(\be,\be)$
	and $\Wb_\epsilon(\al,\be)\xrightarrow{\epsilon \rightarrow 0}
	\OT_0(\al,\be)$.
\end{prop}

\begin{proof}	
	The result for the case $\epsilon \rightarrow 0$ follows
	from~\cite{leonard2012schrodinger,Carlier2017},
	in which the authors show that 
	$\W_\epsilon(\al,\be)\rightarrow \OT_0(\al,\be)$
	for all $\al$ and $\be$ 
  The second limit is a consequence of
  Proposition~\ref{prop:remarkable_potentials}
  (Remarkable values of $\W_\epsilon$ and its dual potentials).
  
  
  Please note that a similar proposition was proved
  in~\cite{genevay2018learning} (following ideas
  from~\cite{RamdasSinkhAsymptotics}) 
  using a ``sharp'' OT cost $\langle\pi_\epsilon,\C\rangle$,
  with $\pi_\epsilon$ the solution of~\eqref{eq-primal-ot}, 
  instead of the full regularized cost
  $\OT_\epsilon(\al,\be)=\langle\pi_\epsilon,\C\rangle
  + \epsilon\,\KL(\pi_\epsilon,\al\otimes\be)$.
\end{proof} 


	

